Failure-Aware Multi-Robot Coordination for Resilient and Adaptive Target Tracking

Multi-robot coordination is crucial for autonomous systems, yet real-world deployments often encounter various failures. These include both temporary and permanent disruptions in sensing and communication, which can significantly degrade system robustness and performance if not explicitly modeled. Despite its practical importance, failure-aware coordination remains underexplored in the literature. To bridge the gap between idealized conditions and the complexities of real-world environments, we propose a unified failure-aware coordination framework designed to enable resilient and adaptive multi-robot target tracking under both temporary and permanent failure conditions. Our approach systematically distinguishes between two classes of failures: (1) probabilistic and temporary disruptions, where robots recover from intermittent sensing or communication losses by dynamically adapting paths and avoiding inferred danger zones, and (2) permanent failures, where robots lose sensing or communication capabilities irreversibly, requiring sustained, decentralized behavioral adaptation. To handle these scenarios, the robot team is partitioned into subgroups. Robots that remain connected form a communication group and collaboratively plan using partially centralized nonlinear optimization. Robots experiencing permanent disconnection or failure continue to operate independently through decentralized or individual optimization, allowing them to contribute to the task within their local context. We extensively evaluate our method across a range of benchmark variations and conduct a comprehensive assessment under diverse real-world failure scenarios. Results show that our framework consistently achieves robust performance in realistic environments with unknown danger zones, offering a practical and generalizable solution for the multi-robot systems community.

==> bib.tex <==
@inproceedings{bartolomei2020perception,
  title={Perception-aware path planning for uavs using semantic segmentation},
  author={Bartolomei, Luca and Teixeira, Lucas and Chli, Margarita},
  booktitle={2020 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={5808--5815},
  year={2020},
  organization={IEEE}
}


@article{wu2022perception,
  title={Perception-aware receding horizon trajectory planning for multicopters with visual-inertial odometry},
  author={Wu, Xiangyu and Chen, Shuxiao and Sreenath, Koushil and Mueller, Mark W},
  journal={IEEE Access},
  volume={10},
  pages={87911--87922},
  year={2022},
  publisher={IEEE}
}

@inproceedings{guo2019safe,
  title={Safe path planning with gaussian process regulated risk map},
  author={Guo, Hongliang and Meng, Zehui and Huang, Zefan and Kang, Leong Wei and Chen, Ziyue and Meghjani, Malika and Ang, Marcelo and Rus, Daniela},
  booktitle={2019 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={2044--2051},
  year={2019},
  organization={IEEE}
}

@article{zhou2011multirobot,
  title={Multirobot active target tracking with combinations of relative observations},
  author={Zhou, Ke and Roumeliotis, Stergios I},
  journal={IEEE Transactions on Robotics},
  volume={27},
  number={4},
  pages={678--695},
  year={2011},
  publisher={IEEE}
}

@inproceedings{schwager2017multi,
  title={A multi-robot control policy for information gathering in the presence of unknown hazards},
  author={Schwager, Mac and Dames, Philip and Rus, Daniela and Kumar, Vijay},
  booktitle={Robotics Research: The 15th International Symposium ISRR},
  pages={455--472},
  year={2017},
  organization={Springer}
}



